Suppression of Recurrence in the Hermite-Spectral Method for Transport Equations

We study the unphysical recurrence phenomenon arising in the numerical simulation of the transport equations using Hermite-spectral method. From a mathematical point of view, the suppression of this numerical artifact with filters is theoretically analyzed for two types of transport equations. It is rigorously proven that all the non-constant modes are damped exponentially by the filters in both models, and formally shown that the filter does not affect the damping rate of the electric energy in the linear Landau damping problem. Numerical tests are performed to show the effect of the filters.

==> article_filter.tex <==
\section{Filtered hyperbolic moment method}\label{sec:FilterHME}
As is discussed in the introduction, filtering is a common procedure
to reduce the effects of the Gibbs phenomenon in spectral methods for
numerical solution of partial differential equations
\cite{canuto2012spectral}. In Section \ref{sec:HME}, we pointed out
that the hyperbolic moment method can be treated as an ``adaptive''
Hermite collocation method on the Vlasov equation, thus it would be
natural to apply a filter on the hyperbolic moment method. In
\cite{Cheng}, Cheng and Knorr showed the filamentation has little
influence on the lower moments of the distribution function in many
cases. It is expected the filter can remove the filamentation but only
slightly affect the macroscopic phenomenon, for example Landau
damping. In this section, we investigate the filter method on the HME.

\subsection{Filter method}
At the first step, we study necessary conditions for the filter. Below
we are going to give two version of filters. The first version is the
classical Hou-Li's \cite{hou2007computing} filter.  However, for this
kind of filter, if the time step is halved, the effect of the filter
changes due to the filter applied twice in the original one time step.
Noticing this deficiency, we proposed the second version of the
filter, which takes the time step into considerison.
\subsubsection{Necessary conditions of the filter}
The usual practice of the filter for spectral method
\cite{parker2015fourier, mcclarren2010robust} is multiplying the
spectral coefficients by the filter factor $\sigma_M(\balpha)$. For
HME, the coefficients $f_{\balpha}$ are corresponding spectral
coefficients, thus the filter can be written as
\begin{equation}
    \tilde{f}_{\balpha} := f_{\balpha}\sigma_M(\balpha).
\end{equation}
And accordingly, the distribution function is replaced by 
\begin{equation}\label{eq:filtered_distribution}
    \sigma(f):=\tilde{f}=\sum_{|\alpha|\leq M}\tilde{f}_{\balpha}
    \mH^{[\bu(t,\bx),u_{th}(t,x)]}_{\alpha}(\bv).
\end{equation}
It is an important issue to choose the filter. Before it, we delineate
the necessary conditions for the filter.

Since HME is a physical model, satisfying the Galealian
transformation invariance, the filte should preserve the Galealian 
transformation invariance of the model, including the rotational
invariance. Hence, we demand the rotational invariance of the
filter, i.e
\begin{equation}\label{eq:filter_rotational}
    \sigma_M(\balpha)=\sigma_M(|\balpha|),\quad |\balpha|\leq M.
\end{equation}
The filter is used to remove the filamentation, which is caused by
high frequency coefficients. Hence, the filter should be stronger for
higher frequency coefficients, i.e. the filter is a monotone
decreasing function.  Here $\balpha$ is a multi-index, so there are
various definition of the monotone decreasing. Due to the rotational
invariance relation
\eqref{eq:filter_rotational}, we let
\begin{equation}\label{eq:filter_monotone}
    \sigma_M(|\balpha|)\geq \sigma_M(|\balpha|+1),\quad |\balpha|<M.
\end{equation}
As the order $M$ increasing, the filtered distribution
\eqref{eq:filtered_distribution} should convergent to the
distribution, which is necessary condition for the convergence of the
model. So for any given $\balpha\in\bbN^D$, the strength of the
filter should vanish, so we have
\begin{equation}\label{eq:filter_limit}
    \lim_{M\rightarrow\infty}\sigma_M(\balpha)=1.
\end{equation}
The conservation of mass, momentum and energy are primary properties
of the VP system. Thus a good filter is expected to preserve the
conservation. Here we demand
\begin{equation}\label{eq:filter_conservation}
    \sigma_M(\alpha)=1,\quad |\alpha|\leq M_0.
\end{equation}
The conservation of mass, momentum and energy demand $M_0\geq 2$.

All the conditions \eqref{eq:filter_rotational},
\eqref{eq:filter_monotone}, \eqref{eq:filter_limit} and
\eqref{eq:filter_conservation} are necessary conditions for the
filter. Next we are trying to find the filter based on these conditions. 
\subsubsection{Hou-Li' filter}
\note{More argument}{briefly review the filter in literatures. rewrite
this subsubsection after the introduction}
In \cite{hou2007computing}, the authors proposed a filter for Fourier
spectral method, which reads
\begin{equation}\label{eq:houli_filter}
    \sigma_N(k) = \left\{ \begin{array}{ll}
        1,&\text{ if } |k|/N\leq 2/3,\\
        \exp(-\beta(|k|/N)^\gamma),& \text{ if } |k|/N>2/3,
    \end{array} \right.
\end{equation}
where $\beta=36$ and $\gamma=36$, which subjects to $\sigma_N(N)$
close to machine precision $2^{-53}$. This filter achieved great
success in
Fourier spectral method \cite{hou2007computing, hou2008numerical}, and
was also used in Fourier-Hermite spectral method for Landau damping
\cite{parker2015fourier}. Moreover, this filter also satisfies the
condition \eqref{eq:filter_monotone}, \eqref{eq:filter_limit} and
\eqref{eq:filter_conservation}, and the rotational invariance relation
\eqref{eq:filter_rotational} can be easy to satisfied by careful
extension to $D$-dimensional case. A natural extension of 
\eqref{eq:houli_filter} is
\begin{equation}\label{eq:filter}
    \sigma_M(\balpha)=\left\{ \begin{array}{ll}
        1,&\text{ if } |\balpha|/M\leq 2/3,\\
        \exp(-\beta(|\balpha|/M)^\gamma), &
        \text{ if } |\balpha|/M>2/3.
    \end{array} \right.
\end{equation}
Easy to check all the four conditions \eqref{eq:filter_rotational},
\eqref{eq:filter_monotone}, \eqref{eq:filter_limit} and
\eqref{eq:filter_conservation} are satisfied. For the parameters
$\beta$ and $\gamma$, it is natural to set them same as those in
\eqref{eq:houli_filter}.

The filter will be applied on the solution after each time step. The
outline of the algorithm can be summerized as
\begin{enumerate}
    \item  Set $n=0$, $t=0$, give order $M$ and the initial value on the
        $i$-th mesh cell $f_{i,\balpha}^n$, $\bu_i^n$ and
        $\bu_{th,i}^n$;
    \item  Calculate the time step length $\Delta t^n$ according to
      the CFL condition;
  \item  Use the numerical scheme in \cite{NRxxVlasov2012} to
      solve the Vlasov equation \eqref{eq:vlasov} by one time step,
      and denote the solution in $i$-th mesh cell as 
      $f_{i,\balpha}^{n,*}$, $\bu_i^{n,*}$ and
      $u_{th,i}^{n,*}$;
  \item $f_{i,\balpha}^{n+1}\leftarrow
      \sigma_M(\balpha)f_{i,\balpha}^{n,*}$,
      $\bu_i^{n+1}\leftarrow \bu_i^{n,*}$,
      $u_{th,i}^{n+1}\leftarrow u_{th,i}^{n,*}$;
    \item Let $n \leftarrow n+1$, $t\leftarrow t+\Delta t^n$ till
        $t\geq t_{end}$.
\end{enumerate}
We refer the readers to the Section 3 of \cite{NRxxVlasov2012} for the
details of the CFL condition and the numerical scheme in the outline
of the algorithm.

\subsubsection{Time step dependent filter}
Since the filter is applied on the distribution function after each
time step, for a given space discretization and a given truncated
order $M$, the time step is chosen as $\Delta t=dt$, then in the time
interval $[t^n, t^n+dt)$, the filter is applied once on the
distribution functions. If the time step is halved as $\Delta t =
dt/2$, then the filter is applied twice in the time interval $[t^n,
t^n+dt)$. If the time step approaches $dt$ to zero, the filter is
applied infinite times in the time interval $[t^n,t^n+dt)$. In this
sense, the effect of the filter \eqref{eq:houli_filter} is close to
the cut-off filter 
\begin{equation}\label{eq:cutoff_filter}
    \sigma_N^{cut}(k)=\left\{ \begin{array}{ll}
        1,  & \text{ if } |k|/N\leq 2/3,\\
        0,  & \text{ if } |k|/N>2/3.
    \end{array} \right.
\end{equation}
In other words, the filter \eqref{eq:filter} is sensitive to the time
step. The effect of the filter strengthens as the time step
decreasing. Hence, different time step may result in different
numerical results, even though with same numrical scheme and same
space and velocity space discretization. To overcome this flaw, the
time step should be considered in the filter.

Denote the semi-discrete scheme with respect to $t$ of the VP equation by 
\begin{equation}\label{eq:filter_VP}
    f^{n,*}=f^{n}+\Delta t\mL(f^n).
\end{equation}
Then applying the filter \eqref{eq:filter} on it, we obtain 
\begin{equation}\label{eq:fonce}
    f^{n+1}_1 := \sigma(f^{n,*}) = \sigma_{\Delta t}(f^n)+\Delta t \sigma_{\Delta t}(\mL(f^n)).
\end{equation}
Here that $\sigma_{\Delta t}(\cdot)$ is a linear operator is used.
If the time step is halved, then in the time interval $[t^n,
t^n+\Delta t)$, the filter is applied twice, and the result is 
\begin{equation}\label{eq:ftwice}
    \begin{aligned}
        \tilde{f}^{n} &:= \sigma_{\Delta t/2}(f^n)+\frac{\Delta t}{2}
        \sigma_{\Delta t/2}(\mL(f^n)),\\
        f^{n+1}_2&:=\sigma_{\Delta t/2}(\tilde{f}^n)
        +\frac{\Delta t}{2}\sigma_{\Delta t/2}(\mL(\tilde{f}_n)),\\
        &\: =\sigma_{\Delta t/2}(\sigma_{\Delta t/2}(f^n))
        +\Delta t\sigma_{\Delta t/2}(\sigma_{\Delta t/2}(\mL(f^n)))
        +O(\Delta t^2),
    \end{aligned}
\end{equation}
where we assume $\Delta t$ is small enough.
Comparing \eqref{eq:fonce} and \eqref{eq:ftwice}, it is natural to
choose the filter such that
\begin{equation}\label{eq:timedependent}
    \sigma_{\Delta t}(f^n)= \sigma_{\Delta t/2}(\sigma_{\Delta t/2}(f^n))
    +O(\Delta t^2).
\end{equation}
In this way, the filter is expected to be not sensitive to the time
step. Meanwhile, Hou and Li's filter \eqref{eq:houli_filter} is set
as $\sigma_N(N)$ reaching the machine precision
\cite{hou2007computing}, which indicates the highest frequency
are always set to zero. Since the recurrence phenomenon is caused by
the high frequency oscillation in the distribution, we expect the
strength of the filter on the highest frequency as strong as possible.
So we plan to keep the property that $\sigma_N(N)$ reaches the machine
precision. Taking these in considerison, we choose the filter as
\begin{equation} \label{eq:filter_t}
    \sigma_M^t(\balpha,\Delta t) = \left\{ \begin{array}{ll}
        1,&\text{ if } |\alpha|/M\leq 2/3,\\
        \exp(-\beta (|\alpha|/M)^\gamma g(\balpha,\Delta t) ),
        &\text{ if } |\alpha|/M > 2/3,
    \end{array} \right.
\end{equation}
where
\begin{equation} \label{eq:filter_factor}
    \beta = 36, \quad \gamma=36,\quad 
    g(\balpha,\Delta t) = \left( \frac{\Delta t}{\Delta t_0}
    \right)^{1-(|\alpha|/M)^\gamma}.
\end{equation}
Here $\Delta t_0$ is a reference time step, which depends on the
problem.

\begin{figure}[ht]
    \centering
    \subfigure[$M=30$]{
        \includegraphics[width=.3\textwidth]{filter_30_c.eps}
    }
    \subfigure[$M=90$]{
        \includegraphics[width=.3\textwidth]{filter_90_c.eps}
    }
    \subfigure[$M=300$]{
        \includegraphics[width=.3\textwidth]{filter_300_c.eps}
    }
    \caption{\label{fig:filter}Profile of the filter
    \eqref{eq:filter_t} with different $\Delta t/\Delta t_0$ and the
    order $M$. The $x$ and $y$ axis are $|\balpha|$ and
    $\sigma_M^t(\balpha,\Delta t)$, respectively, and the legend is
for the values of $\Delta t/\Delta t_0$.}
\end{figure}

For the highest frequencies, i.e $|\balpha|/M\sim 1$,
$g(\balpha,\Delta t)\sim 1$, so $\sigma_M^t(\balpha,\Delta)$ are close
to the machine precision. Otherwise, $g(\alpha,\Delta t)\sim
\frac{\Delta t}{\Delta t_0}$, the relation \eqref{eq:timedependent}
valids.
Moreover, when $\balpha|/M\sim 1$, $\sigma_M^t(\balpha, \Delta t)$ is
close to $0$, thus we have $\sigma_M^t(\balpha, \Delta
t)f_{\alpha}=o(\Delta t^2)$, i.e \eqref{eq:timedependent} is also
valid.
And easy to check the filter \eqref{eq:filter_t}
satisfies all the four conditions \eqref{eq:filter_rotational},
\eqref{eq:filter_monotone}, \eqref{eq:filter_limit} and
\eqref{eq:filter_conservation}.
Fig. \ref{fig:filter} gives the time step filter \eqref{eq:filter_t}
with different $M$ and different relative time step $\Delta t/\Delta
t_0$. And the case $\Delta t/\Delta t_0=1$ corresponds to the filter
\eqref{eq:filter}.

\subsection{Collision viewpoint}


==> article_todo.tex <==
\section{Conclusion}
In summary, ...
%the hyperbolic moment system has been derived for the 
%Vlasov-Maxwell equations. We have proven that the moment method conserves
%charge, conserves momentum, conserves energy and is stable. The corresponding
%numerical method is developing for the moment system obtained, and will be 
%apply to study important plasma physics problems in the future.
\begin{enumerate}
    \item 解释滤波器对电场能衰减速率和震荡频率的影响都很小
    \item $t>150$ 后，电场能大小为 $N \mu$，其中 $N$ 为网格数， $\mu$ 为机器精度。
        \item 说明滤波器不改变 Landau 阻尼电场能衰减率时。
            从三个角度说，
            首先说明在未出现 recurrence 之前和没有滤波器前的情况几乎一样；
            其次，
            说明出现之后，
            加入滤波器所得的衰减速率能和之前的结果几乎一样。
            最后说明在极限意义下，加入滤波器的结果和衰减速率的理论解可以一致。
            这个就涉及到矩数和网格剖分方向的收敛性了。
			\item $k=0.2,0.3,0.4$ 的情况还未计算。
			\item 对比未加 filter 和加入 filter 以后算的最好的参数。
			\item 未出现 recurrence 之前加不加 filter 的局部放大图。
			说明加入 filter 以后，没有出现 recurrence 时，
			和 HME 的结果几乎一样。
			\item 用图说明加密空间网格对于数值结果的影响并不大。
\end{enumerate}

\section*{Acknowledgements} This research of Y. Di is supported in
part by the Natural Science Foundation of China No. 11271358. 
%R. Li is supported in part by
%the National Basic Research Program of China (2011CB309704) and the
%National Natural Science Foundation of China No. 11325102 and No.
%91330205.


